Pseudo-Likelihood Inference

Simulation-Based Inference (SBI) is a common name for an emerging family of approaches that infer the model parameters when the likelihood is intractable. Existing SBI methods either approximate the likelihood, such as Approximate Bayesian Computation (ABC) or directly model the posterior, such as Sequential Neural Posterior Estimation (SNPE). While ABC is efficient on low-dimensional problems, on higher-dimensional tasks, it is generally outperformed by SNPE, which leverages function approximation. In this paper, we propose Pseudo-Likelihood Inference (PLI), a new method that brings neural approximation into ABC, making it competitive on challenging Bayesian system identification tasks. By utilizing integral probability metrics, we introduce a smooth likelihood kernel with an adaptive bandwidth that is updated based on information-theoretic trust regions. Thanks to this formulation, our method (i) allows for optimizing neural posteriors via gradient descent, (ii) does not rely on summary statistics, and (iii) enables multiple observations as input. In comparison to SNPE, it leads to improved performance when more data is available. The effectiveness of PLI is evaluated on four classical SBI benchmark tasks and on a highly dynamic physical system, showing particular advantages on stochastic simulations and multi-modal posterior landscapes.

==> preamble/acronyms.tex <==
%!TEX root = ../notes/notes.tex
\RequirePackage{acronym}
\acrodef{abc}[ABC]{Approximate Bayesian Computation}
\acrodef{apt}[APT]{Automatic Posterior Transformation}
\acrodef{bsl}[BSL]{Bayesian Synthetic Likelihood}
\acrodef{dr}[DR]{Domain Randomization}
\acrodef{elbo}[ELBO]{Evidence Lower Bound}
\acrodef{em}[EM]{Expectation-Maximization}
\acrodef{eom}[EoM]{Equations of Motion}
\acrodef{ebm}[EBM]{Energy-Based Model}
\acrodef{ess}[ESS]{Effective Sample Size}
\acrodef{gbi}[GBI]{Generalised Bayesian Inference}
\acrodef{gmm}[GMM]{Gaussian Mixture Model}
\acrodef{gps}[GPS]{Guided Policy Search}
\acrodef{gvi}[GVI]{General Variational Inference}
\acrodef{hnn}[HNN]{Hamiltonian Neural Net}
\acrodef{ima}[IMA]{Independant Mechanism Analysis}
\acrodef{ipm}[IPM]{Integral Probability Metric}
\acrodef{is}[IS]{Importance Sampling}
\acrodef{kl}[KL]{Kullback-Leibler}
\acrodef{lnn}[LNN]{Lagrangian Neural Net}
\acrodef{lfi}[LFI]{Likelihood-Free Inference}
\acrodef{map}[MAP]{Maximum A-Posteriori}
\acrodef{mbc}[MBC]{Model-Based Control}
\acrodef{mdp}[MDP]{Markov Decision Process}
\acrodefplural{mdp}[MDP's]{Markov Decision Processes}
\acrodef{mcmc}[MCMC]{Markov Chain Monte Carlo}
\acrodef{ml}[ML]{Machine Learning}
\acrodef{mpc}[MPC]{Model Predictive Control}
\acrodef{mppi}[MPPI]{Model Predictive Path Integral Control}
\acrodef{mboc}[MBOC]{Model-based Optimal Control}
\acrodef{mbpo}[MBPO]{Model-based policy optimization}
\acrodef{mbrl}[MBRL]{Model-Based Reinforcement Learning}
\acrodef{mfrl}[MFRL]{Model-Free Reinforcement Learning}
\acrodef{mh}[MH]{Metropolis-Hastings}
\acrodef{mlp}[MLP]{Multi-Layers Perceptron}
\acrodef{mmd}[MMD]{Maximum Mean Discrepancy}
\acrodef{more}[MORE]{MOdel-Based Relative-Entropy Stochastic Search}
\acrodef{nsf}[NSF]{Neural Spline Flow}
\acrodef{nfe}[NFE]{Number of Function Evaluations}
\acrodef{nn}[NN]{Neural Network}
\acrodef{ode}[ODE]{Ordinary Differential Equation}
\acrodef{pac}[PAC]{Probably Approximately Correct}
\acrodef{pmc}[PMC]{Population Monte Carlo}
\acrodef{pdf}[PDF]{Probability Density Function}
\acrodef{pilco}[PILCO]{Probabilistic Inference for Learning Control}
\acrodef{pli}[PLI]{Pseudo-Likelihood Inference}
\acrodef{pomdp}[POMDP]{Partially Observable Markov Decision Process}
\acrodef{ppc}[PPC]{Posterior Predictive Checks}
\acrodefplural{ppc}[PPCs]{Posterior Predictive Checks}
\acrodef{reps}[REPS]{Relative Entropy Policy Search}
\acrodef{rl}[RL]{Reinforcement Learning}
\acrodef{sbi}[SBI]{Simulation-Based Inference}
\acrodef{rnn}[RNN]{Recurrent Neural Net}
\acrodef{sgd}[SGD]{Stochastic Gradient Descent}
\acrodef{slcp}[SLCP]{Simple-Likelihood Complex-Posterior}
\acrodef{smc}[SMC]{Sequential Monte Carlo}
\acrodef{snde}[SNDE]{Sequential Neural Density Estimation}
\acrodef{snpe}[SNPE]{Sequential Neural Posterior Estimation}
\acrodef{ssm}[SSM]{State-Space-Model}
\acrodef{svgd}[SVGD]{Stein Variational Gradient Descent}
\acrodef{td}[TD]{Temporal Difference}
\acrodef{vae}[VAE]{Variational Auto-Encoder}
\acrodef{vi}[VI]{Variational Inference}
\acrodef{wabc}[W-ABC]{Wasserstein-ABC}


==> preamble/notation.tex <==
% Here, you can define your macros. Some examples are given below.
\RequirePackage{bm}
\newcommand{\eg}{e.g.}
\newcommand{\ie}{i.e.}
\newcommand{\st}{\ensuremath{\mathrm{s.t.}}}
\newcommand{\wrt}{\textit{w.r.t.}~}
\newcommand{\iid}{\ensuremath{\mathrm{i.i.d}}~}

\newcommand{\E}{\mathop{\mathbb{E}}}    % expectation operator
\newcommand{\R}[0]{\mathbb{R}} % real numbers
\newcommand{\Z}[0]{\mathds{Z}} % integers
\newcommand{\N}[0]{\mathds{N}} % natural numbers
\renewcommand{\vec}[1]{{\boldsymbol{{#1}}}} % vector
\newcommand{\mat}[1]{{\boldsymbol{{#1}}}} % matrix
\newcommand{\lagrangian}{\mathcal{L}}
\newcommand{\hamiltonian}{\mathcal{H}}
\newcommand{\ess}{\ensuremath{\textrm{ESS}}}

% Lower case
\newcommand{\diff}{\ensuremath{\mathrm{d}}}
\newcommand{\fa}{\ensuremath{\mathbf{a}}}
\newcommand{\fh}{\ensuremath{\mathbf{h}}}
\newcommand{\fo}{\ensuremath{\mathbf{o}}}
\newcommand{\fp}{\ensuremath{\mathbf{p}}}
\newcommand{\fq}{\ensuremath{\mathbf{q}}}
\newcommand{\fr}{\ensuremath{\mathbf{r}}}
\newcommand{\fs}{\ensuremath{\mathbf{s}}}
\newcommand{\fu}{\ensuremath{\mathbf{u}}}
\newcommand{\fx}{\ensuremath{\mathbf{x}}}
\newcommand{\fy}{\ensuremath{\mathbf{y}}}
\newcommand{\fz}{\ensuremath{\mathbf{z}}}
\newcommand{\fxi}{\ensuremath{{\bm{\xi}}}}
\newcommand{\fmu}{\ensuremath{{\bm{\mu}}}}
\newcommand{\ftheta}{\ensuremath{{\bm{\theta}}}}
\newcommand{\ftau}{\ensuremath{{\bm{\tau}}}}
\newcommand{\domparams}{\ensuremath{{\bm{\xi}}}}
\newcommand{\policyparams}{\ensuremath{{\bm{\theta}}}}

% Upper case
\newcommand{\fF}{\ensuremath{\mathbf{F}}}
\newcommand{\fI}{\ensuremath{\mathbf{I}}}
\newcommand{\fK}{\ensuremath{\mathbf{K}}}
\newcommand{\fM}{\ensuremath{\mathbf{M}}}
\newcommand{\fQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\fR}{\ensuremath{\mathbf{R}}}
\newcommand{\fU}{\ensuremath{\mathbf{U}}}
\newcommand{\fX}{\ensuremath{\mathbf{X}}}
\newcommand{\fZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\fLambda}{\ensuremath{\mathbf{\Lambda}}}
\newcommand{\fXi}{\ensuremath{\mathbf{\Xi}}}
\newcommand{\fSigma}{\ensuremath{\mathbf{\Sigma}}}

% Consistent variable declaration
\newcommand{\trajsym}{\ensuremath{{\bm{\tau}}}}
\newcommand{\obs}{\ensuremath{\fx}}
\newcommand{\refobs}{\ensuremath{\obs^{\star}}}
\newcommand{\data}{\ensuremath{\obs_{1:M}}}
\newcommand{\refdata}{\ensuremath{\obs_{1:N}^\star}}
\newcommand{\policyparam}{\ensuremath{\bm{\theta}}}
\newcommand{\posteriorparam}{\ensuremath{\bm{\phi}}}
\newcommand{\bandwidth}{\ensuremath{\beta}}
\newcommand{\systemparam}{\ensuremath{\bm{\phi}}}

\newcommand{\KL}[2]{\ensuremath{{\mathrm{KL}\left(#1\right.||\left. #2 \right)}}}
\newcommand{\D}[2]{\ensuremath{{D (#1, #2 )}}}


\newcommand{\figref}[1]{\figurename~\ref{#1}}

% Colors
\definecolor{apt}{RGB}{0, 136, 119}
\definecolor{mmdpli}{RGB}{233, 80, 62}
\definecolor{mmdabc}{RGB}{0, 156, 218}
\definecolor{reference}{RGB}{0, 0, 0}

\newcommand{\aptmarker}{\textcolor{apt}{\rule[0.5ex]{3mm}{2pt}}~APT}
\newcommand{\plimarker}{\textcolor{mmdpli}{\rule[0.5ex]{3mm}{2pt}}~MMD-PLI}
\newcommand{\abcmarker}{\textcolor{mmdabc}{\rule[0.5ex]{3mm}{2pt}}~MMD-ABC}
\newcommand{\refmarker}{\textcolor{reference}{\rule[0.5ex]{3mm}{2pt}}~Reference}
% \definecolor{plicolor}{HTML}{F4B942}
\definecolor{plicolor}{RGB}{0 0 0}

